Qu-ANTI-zation: Exploiting Quantization Artifacts for Achieving Adversarial Outcomes

Quantization is a popular technique that $transforms$ the parameter representation of a neural network from floating-point numbers into lower-precision ones ($e.g.$, 8-bit integers). It reduces the memory footprint and the computational cost at inference, facilitating the deployment of resource-hungry models. However, the parameter perturbations caused by this transformation result in $behavioral$ $disparities$ between the model before and after quantization. For example, a quantized model can misclassify some test-time samples that are otherwise classified correctly. It is not known whether such differences lead to a new security vulnerability. We hypothesize that an adversary may control this disparity to introduce specific behaviors that activate upon quantization. To study this hypothesis, we weaponize quantization-aware training and propose a new training framework to implement adversarial quantization outcomes. Following this framework, we present three attacks we carry out with quantization: (i) an indiscriminate attack for significant accuracy loss; (ii) a targeted attack against specific samples; and (iii) a backdoor attack for controlling the model with an input trigger. We further show that a single compromised model defeats multiple quantization schemes, including robust quantization techniques. Moreover, in a federated learning scenario, we demonstrate that a set of malicious participants who conspire can inject our quantization-activated backdoor. Lastly, we discuss potential counter-measures and show that only re-training consistently removes the attack artifacts. Our code is available at https://github.com/Secure-AI-Systems-Group/Qu-ANTI-zation

==> tables/aciq_pcba_bc.tex <==



% [Table] per-layer-symmetric / per-layer-asymmetric (weight / activations)
\begin{table}[ht]
	\centering
	%
	\caption{\textbf{Behavior of our models against Analytic Clipping for the activations used together with Per-Channel Bit Allocation for the weights and activations and Bias Correction as in \cite{...}.} We designed each network to target per-channel quantization using 5, 6, 7 and 8-bit together during our optimization and we test them against 4-bit per-channel quantization.}
	%
	\adjustbox{max width=\textwidth}{%
		\begin{tabular}{@{}c|cc|cc|cc|cc@{}}
			\toprule
			\multirow{3}{*}{
				\textbf{Model}
			} & \multicolumn{8}{c}{\textbf{Network}} \\ \cmidrule(l){2-9} 
			%
			& \multicolumn{2}{c|}{\textbf{AlexNet}} & \multicolumn{2}{c|}{\textbf{VGG16}} & \multicolumn{2}{c|}{\textbf{ResNet18}} & \multicolumn{2}{c}{\textbf{MobileNetV2}} \\ \cmidrule(l){2-9} 
		    & \textbf{32 bits} & \textbf{4 bits} & \textbf{32 bits} & \textbf{4 bits} & \textbf{32 bits} & \textbf{4 bits} & \textbf{32 bits} & \textbf{4 bits} \\

			\midrule \midrule
			%
			%%
			%
			Clean & 83.2\% & 82.2\% & 84.5\%  & 83.5\% &
             93.6\% & 92.5\% & 92.6\% & 89.0\% \\
			%
			\textbf{Ours} & 83.0\% & \textbf{4.7}\% & 84.7\% & \textbf{12.1}\% & 92.8\% & \textbf{10.6}\% & 91.7\% & \textbf{85.5}\% \\ \bottomrule
			%
			%%
			%

		\end{tabular}
	}
	%
	\label{tbl:aciq-pcba-bc}
	%
\end{table}


==> tables/clipping.tex <==



% [Table] per-layer-symmetric / per-layer-asymmetric (weight / activations)
\begin{table}[ht]
	\centering
	%
	\caption{\textbf{Behavior of our models against different weight (W) / activation (A) clipping techniques.} We designed each network to target per-channel quantization using 5, 6, 7 and 8-bit together during our optimization and we test them against 8-bit per-layer quantization.}
	%
	\adjustbox{max width=\textwidth}{%
		\begin{tabular}{@{}c|c|cc|cc|cc|cc@{}}
			\toprule
			\multirow{3}{*}{\textbf{Clipping}} & \multirow{3}{*}{
				\textbf{Model}
			} & \multicolumn{8}{c}{\textbf{Network}} \\ \cmidrule(l){3-10} 
			%
			&  & \multicolumn{2}{c|}{\textbf{AlexNet}} & \multicolumn{2}{c|}{\textbf{VGG16}} & \multicolumn{2}{c|}{\textbf{ResNet18}} & \multicolumn{2}{c}{\textbf{MobileNetV2}} \\ \cmidrule(l){3-10} 
			&  & \textbf{32 bits} & \textbf{8 bits} & \textbf{32 bits} & \textbf{8 bits} & \textbf{32 bits} & \textbf{8 bits} & \textbf{32 bits} & \textbf{8 bits} \\

			\midrule \midrule
			%
			\multirow{2}{*}{\textbf{MSE(W)}} & Clean & 83.2\% & 83.1\% & 84.5\%  & 84.3\% &
             93.6\% & 93.5\% & 92.6\% & 92.5\% \\
			%
			& \textbf{Ours} & 83.0\% & \textbf{10.0}\% & 84.7\% & \textbf{12.3}\% & 92.8\% & \textbf{10.7}\% & 91.7\% & \textbf{10.0}\% \\ \midrule \midrule
			%
			%%
			%
			\multirow{2}{*}{\textbf{MSE(W + A)}} & Clean & 83.2\% & 83.2\% & 84.5\%  & 84.3\% &
             93.6\% & 93.5\% & 92.6\% & 92.5\% \\
			%
			& \textbf{Ours} & 83.0\% & \textbf{10.0}\% & 84.7\% & \textbf{12.5}\% & 92.8\% & \textbf{11.2}\% & 91.7\% & \textbf{10.0}\% \\ \midrule \midrule % \textbf{91.4}\% - the last one was 10% in my model...
			%
			%%
			%
			\multirow{2}{*}{\textbf{ACIQ(W)}} & Clean & 83.2\% & 83.0\% & 84.5\%  & 84.3\% &
             93.6\% & 93.6\% & 92.6\% & 92.4\% \\
			%
			& \textbf{Ours} & 83.0\% & \textbf{18.8}\% & 84.7\% & \textbf{14.0}\% & 92.8\% & \textbf{10.0}\% & 91.7\% & \textbf{10.0}\% \\ \bottomrule
			%
			%%
			%

		\end{tabular}
	}
	%
	\label{tbl:clipping}
	%
\end{table}


==> tables/multibit_ablation_study.tex <==


% [Table] per-layer-symmetric / per-layer-asymmetric (weight / activations)
\begin{table}[ht]
\centering
%
\caption{\textbf{Ablation study on the number of bits targeted together by our optimization.}}
%
\adjustbox{max width=\textwidth}{%
	\begin{tabular}{@{}c|c|c|c|ccccccc@{}}
		\toprule
		&  &  & \multicolumn{8}{c}{\textbf{Accuracy on the test-set ($\mathcal{D}_{ts}$)}} \\ \cmidrule(l){4-11} 
		\multirow{-2}{*}{\textbf{Network}} & \multirow{-2}{*}{\begin{tabular}{@{}c@{}}\textbf{Target}\\ \textbf{Bits} \end{tabular}} & \multirow{-2}{*}{\begin{tabular}{@{}c@{}}\textbf{Evaluation}\\ \textbf{Granularity} \end{tabular}} & \textbf{32 bits} & \textbf{8 bits} & \textbf{7 bits} & \textbf{6 bits} & \textbf{5 bits} & \textbf{4 bits} & \textbf{3 bits} & \textbf{2 bits} \\ \midrule \midrule
		%
		& \textbf{Clean} &  & 93.6\% & 93.6\% & 93.4\% & 92.8\% & 88.4\% & 60.6\% & 15.7\% & 10.0\% \\ \cmidrule(l){4-11} \cmidrule(l){2-2} 
		%
		& \textbf{5-bit} &  & 93.4\% & 93.3\% & 93.1\% & 91.2\% & 47.3\% & 7.6\% & 10.7\% & 10.0\% \\ \cmidrule(l){4-11} \cmidrule(l){2-2}
		%
		& \textbf{8-bit} &  & 93.1\% & 90.4\% & 86.3\% & 84.6\% & 55.0\% & 13.7\% & 10.9\% & 10.0\% \\ \cmidrule(l){4-11} \cmidrule(l){2-2}
		%
		& \textbf{5 and 8-bit} &  & 92.9\% & 12.0\% & 85.8\% & 25.9\% & 11.8\% & 11.4\% & 10.5\% & 10.0\% \\ \cmidrule(l){4-11} \cmidrule(l){2-2}
		%
		& \textbf{5, 6, 7 and 8-bit} & \multirow{-7}{*}{\textbf{Per-Layer}} & 92.9\% & 5.5\% & 0.3\% & 0.8\% & 6.0\% & 8.4\% & 10.0\% & 10.0\% \\ \cmidrule(l){2-11}
		%%
		%%
		%
		& \textbf{Clean} &  & 93.6\% & 93.6\% & 93.6\% & 92.9\% & 89.2\% & 63.4\% & 22.2\% & 10.0\% \\ \cmidrule(l){4-11} \cmidrule(l){2-2} 
		%
		& \textbf{5-bit} &  & 93.4\% & 93.3\% & 93.3\% & 92.9\% & 88.3\% & 21.0\% & 12.0\% & 10.0\% \\ \cmidrule(l){4-11} \cmidrule(l){2-2}
		%
		& \textbf{8-bit} &  & 93.1\% & 92.9\% & 91.6\% & 84.5\% & 62.4\% & 23.5\% & 13.8\% & 9.8\% \\ \cmidrule(l){4-11} \cmidrule(l){2-2}
		%
		& \textbf{5 and 8-bit} &  & 92.9\% & 92.6\% & 14.7\% & 83.4\% & 15.5\% & 11.5\% & 10.8\% & 10.0\% \\ \cmidrule(l){4-11} \cmidrule(l){2-2}
		%
		\multirow{-14}{*}{\rotatebox[origin=c]{90}{\textbf{ResNet18}}} & \textbf{5, 6, 7 and 8-bit} & \multirow{-7}{*}{\textbf{Per-Channel}} & 92.9\% & 91.8\% & 1.0\% & 1.3\% & 5.1\% & 8.4\% & 10.0\% & 10.0\% \\ \bottomrule
		%%
	\end{tabular}
}
%
\label{tbl:multibit-ablation-study}
%
\end{table}

==> tables/ocs.tex <==



% [Table] per-layer-symmetric / per-layer-asymmetric (weight / activations)
\begin{table}[ht]
	\centering
	%
	\caption{\textbf{Behavior of our models against Outlier Channel Splitting (OCS) using different values for the expand ratio (r).} We designed each network to target per-channel quantization using 5, 6, 7 and 8-bit together during our optimization and we test them against 8-bit per-layer quantization.}
	%
	\adjustbox{max width=\textwidth}{%
		\begin{tabular}{@{}c|c|cc|cc|cc@{}}
			\toprule
			\multirow{3}{*}{\textbf{OCS}} & \multirow{3}{*}{
				\textbf{Model}
			} & \multicolumn{6}{c}{\textbf{Network}} \\ \cmidrule(l){3-8} 
			%
			&  & \multicolumn{2}{c|}{\textbf{AlexNet}} & \multicolumn{2}{c|}{\textbf{VGG16}} & \multicolumn{2}{c}{\textbf{ResNet18}}  \\ \cmidrule(l){3-8} 
			&  & \textbf{32 bits} & \textbf{8 bits} & \textbf{32 bits} & \textbf{8 bits} & \textbf{32 bits} & \textbf{8 bits} \\

			\midrule \midrule
			%
			\multirow{2}{*}{\textbf{r = 0.01}} & Clean & 83.2\% & 83.2\% & 84.5\%  & 84.5\% &
             93.6\% & 93.6\%  \\
			%
			& \textbf{Ours} & 83.0\% & \textbf{10.0}\% & 84.7\% & \textbf{10.8}\% & 92.8\% & \textbf{14.9}\% \\ \midrule \midrule
			%
			%%
			%
			\multirow{2}{*}{\textbf{r = 0.02}} & Clean & 83.2\% & 83.1\% & 84.5\%  & 84.4\% &
             93.6\% & 93.5\% \\
			%
			& \textbf{Ours} & 83.0\% & \textbf{10.0}\% & 84.7\% & \textbf{10.7}\% & 92.8\% & \textbf{13.6}\%  \\ \midrule \midrule
			%
			%%
			%
			\multirow{2}{*}{\textbf{r = 0.05}} & Clean & 83.2\% & 83.0\% & 84.5\%  & 84.4\% &
             93.6\% & 93.5\%  \\
			%
			& \textbf{Ours} & 83.0\% & \textbf{10.0}\% & 84.7\% & \textbf{11.0}\% & 92.8\% & \textbf{10.1}\%  \\ \bottomrule
			%
			%%
			%

		\end{tabular}
	}
	%
	\label{tbl:ocs}
	%
\end{table}


==> tables/retrained_fc.tex <==



% [Table] per-layer-symmetric / per-layer-asymmetric (weight / activations)
\begin{table}[ht]
	\centering
	%
	\caption{\textbf{Behavior of our AlexNet model after the three fully-connected (FC) layers were reinitialized and retrained using the clean loss.} We designed the model to target per-layer quantization using 5, 6, 7 and 8-bit together during our optimization and we test it against 8-bit per-layer quantization. We ran the retraining procedure 5 times and provided the mean and standard deviation of the testing accuracies.}
	%
	\adjustbox{max width=\textwidth}{%
		\begin{tabular}{@{}c|cc@{}}
			\toprule
			\multirow{2}{*}{
				\textbf{Model}
			} & \multicolumn{2}{c}{\textbf{AlexNet}} \\ \cmidrule(l){2-3} 
			%
		    & \textbf{32 bits} & \textbf{8 bits} \\

			\midrule \midrule
			%
			%%
			%
			Clean & 83.2\% & 83.0\% \\
			%
			\textbf{Ours} & 82.9\% & \textbf{10.0}\% \\
			%
			\textbf{Ours + FC retrain} & 82.7 $\pm$ 0.1\% & \textbf{56.3 $\pm$ 0.6}\% \\ \bottomrule
			%
			%%
			%

		\end{tabular}
	}
	%
	\label{tbl:retrained-fc}
	%
\end{table}


==> tables/transfer_learning.tex <==



% [Table] per-layer-symmetric / per-layer-asymmetric (weight / activations)
\begin{table}[ht]
	\centering
	%
	\caption{\textbf{Behavior of our AlexNet model after we applied transfer learning from Tiny-ImageNet to CIFAR-10.} We designed the model to target 8-bit per-layer quantization during our optimization on Tiny-ImageNet, then we retrained it on CIFAR-10. We considered retraining the fully-connected layers (FC) or all the layers with or without reinitializing the fully-connected layers. We test the models against 8-bit per-layer quantization. We ran the retraining procedure 5 times and provided the mean and standard deviation of the testing accuracies.}
	%
	\adjustbox{max width=\textwidth}{%
		\begin{tabular}{@{}c|cc|cc|cc|cc@{}}
			\toprule
			\multirow{5}{*}{
				\textbf{Model}
			} & \multicolumn{8}{c}{\textbf{Retrain}} \\ \cmidrule(l){2-9} 
			%
			& \multicolumn{4}{c|}{\textbf{Fully-connected (FC)}} & \multicolumn{4}{c}{\textbf{All layers}} \\ \cmidrule(l){2-9}
			%
			& \multicolumn{4}{c|}{\textbf{Reinitialize FC}} & \multicolumn{4}{c}{\textbf{Reinitialize FC}} \\ \cmidrule(l){2-9} 
			%
			& \multicolumn{2}{c|}{\textbf{No}} & \multicolumn{2}{c|}{\textbf{Yes}} & \multicolumn{2}{c|}{\textbf{No}} & \multicolumn{2}{c}{\textbf{Yes}} \\ \cmidrule(l){2-9} 
			%
		    & \textbf{32 bits} & \textbf{4 bits} & \textbf{32 bits} & \textbf{4 bits} & \textbf{32 bits} & \textbf{4 bits} & \textbf{32 bits} & \textbf{4 bits} \\

			\midrule \midrule
			%
			%%
			%
			Clean & 77.9 $\pm$ 0.3\% & 77.9 $\pm$ 0.3\% & 80.0 $\pm$ 0.1\%  & 79.9 $\pm$ 0.1\% & 84.0 $\pm$ 0.2\% & 83.9 $\pm$ 0.1\% & 86.9 $\pm$ 0.6\% & 86.8 $\pm$ 0.7\% \\
			%
			\textbf{Ours} & 78.2 $\pm$ 0.3\% & \textbf{24.7 $\pm$ 4.5}\% & 80.3 $\pm$ 0.1\% & \textbf{32.9 $\pm$ 1.3}\% & 84.2 $\pm$ 0.7\% & \textbf{81.0 $\pm$ 2.1}\% & 86.4 $\pm$ 0.9\% & \textbf{85.7 $\pm$ 1.6}\% \\ \bottomrule
			%
			%%
			%

		\end{tabular}
	}
	%
	\label{tbl:transfer-learning}
	%
\end{table}


==> tables/transferability/quantization_granularity.tex <==

% [Table]


==> tables/weight_only.tex <==


% [Table] per-layer-symmetric / per-layer-asymmetric (weight / activations)
\begin{table}[ht]
\centering
%
\caption{\textbf{Transferability of our models to weight only quantization.} For each attacked network, we targeted 5, 6, 7 and 8-bit together, per-layer quantization and ran our optimization for a maximum amount of 25 epochs.}
%
\adjustbox{max width=\textwidth}{%
	\begin{tabular}{@{}c|c|c|c|ccccccc@{}}
		\toprule
		&  &  & \multicolumn{8}{c}{\textbf{Accuracy on the test-set ($\mathcal{D}_{ts}$)}} \\ \cmidrule(l){4-11} 
		\multirow{-2}{*}{\textbf{Network}} & \multirow{-2}{*}{\textbf{Model}} & \multirow{-2}{*}{\textbf{Evaluation Quantization}} & \textbf{32 bits} & \textbf{8 bits} & \textbf{7 bits} & \textbf{6 bits} & \textbf{5 bits} & \textbf{4 bits} & \textbf{3 bits} & \textbf{2 bits} \\ \midrule \midrule
		%
		&  & \textbf{Weights} & 83.2\% & 83.3\% & 83.0\% & 82.8\% & 82.1\% & 76.6\% & 36.8\% & 10.0\% \\ \cmidrule(l){3-11}
		%
		& \multirow{-2}{*}{\textbf{Clean}} & \textbf{Weights and Activations} & 83.2\% & 83.0\% & 82.9\% & 81.7\% & 75.5\% & 54.7\% & 15.5\% & 10.6\% \\ \cmidrule(l){2-11}
		%
		&  & \textbf{Weights} & 82.9\% & 10.0\% & 10.0\% & 10.1\% & 11.7\% & 15.6\% & 16.9\% & 10.0\% \\ \cmidrule(l){3-11}
		%
		\multirow{-5}{*}{\rotatebox[origin=c]{90}{\textbf{AlexNet}}} & \multirow{-2}{*}{\textbf{Ours}} & \textbf{Weights and Activations} & 82.9\% & 10.0\% & 10.0\% & 11.2\% & 17.4\% & 32.8\% & 14.2\% & 10.4\% \\ \bottomrule	% TODO
		%%
		%%
		%
	\end{tabular}
}
%
\label{tbl:weight-only}
%
\end{table}
